Contextual aggregation and rapid updating of trial outcomes within a user-friendly open-source environment

The delayed and incomplete availability of historical findings and the lack of integrative and user-friendly software hampers the reliable interpretation of new clinical data. We developed a free, open, and user-friendly clinical trial aggregation program combining a large and representative sample of existing trial data with the latest classical and Bayesian meta-analytical models, including clear output visualizations. Our software is of particular interest for (post-graduate) educational programs (e.g., medicine, epidemiology) and global health initiatives. We demonstrate the database, interface, and plot functionality with a recent randomized controlled trial on effective epileptic seizure reduction in children treated for a parasitic brain infection. The single trial data is placed into context and we show how to interpret new results against existing knowledge instantaneously. Our program is of particular interest to those working on the contextualizing of medical findings. It may facilitate the advancement of global clinical progress as efficiently and openly as possible and simulate further bridging clinical data with the latest biostatistical models.

==> tables/simulation_sequential_short.tex <==
\begin{sidewaystable}[ph!]
\caption{Probability (SE) of finding support for the null hypothesis ($H_0$), alternative hypothesis ($H_1$), or not reaching a decision (undecided) in the simulated sequential analysis and the mean time in months (SE) of finding support for either the null or alternative hypothesis for each simulation condition comparing Bayesian model-averaging (BMA) to model selection using information (AIC, BIC), model selection using Bayes factors (BF), excluding the parametric models corresponding to the true data generating process. Results the model selection with AIC /  BIC correspond to k = 20 steps in a sequential analysis with binding asymmetric boundaries, Hwang-Shih-DeCani spending function, and $\alpha = 0.05$ for one-sided test.}
\label{tab:simulation_sequential_short}

\footnotesize
\begin{tabular}{l|rrr|rrr}
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Decision}}} & \multicolumn{3}{c}{log(AF) = -.20} & \multicolumn{3}{|c}{log(AF) = 0} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c}{$H_1$} \\
    \hline
    BMA  & 0.998 (0.002) & 0.000 (0.000) & 0.002 (0.002) & 0.896 (0.014) & 0.048 (0.010) & 0.056 (0.010) \\ 
    BF   & 0.998 (0.002) & 0.000 (0.000) & 0.002 (0.002) & 0.884 (0.014) & 0.056 (0.010) & 0.060 (0.011) \\ 
    AIC  & 1.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.930 (0.011) & 0.042 (0.009) & 0.028 (0.007) \\ 
    BIC  & 1.000 (0.000) & 0.000 (0.000) & 0.000 (0.000) & 0.930 (0.011) & 0.042 (0.009) & 0.028 (0.007)  \\ 
    \hline
    \\
    
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Decision}}} & \multicolumn{3}{c}{log(AF) = 0.20} & \multicolumn{3}{|c}{log(AF) = 0.40} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{Undecided} & \multicolumn{1}{c}{$H_1$} \\
    \hline
    BMA  & 0.184 (0.017) & 0.136 (0.015) & 0.680 (0.021) & 0.016 (0.006) & 0.008 (0.004) & 0.976 (0.007) \\ 
    BF   & 0.164 (0.017) & 0.152 (0.016) & 0.684 (0.021) & 0.016 (0.006) & 0.008 (0.004) & 0.976 (0.007) \\ 
    AIC  & 0.112 (0.014) & 0.212 (0.018) & 0.676 (0.021) & 0.006 (0.003) & 0.012 (0.005) & 0.982 (0.006) \\ 
    BIC  & 0.116 (0.014) & 0.208 (0.018) & 0.676 (0.021) & 0.006 (0.003) & 0.012 (0.005) & 0.982 (0.006) \\ 

    \hline
\end{tabular}
\\
\\

\begin{tabular}{l|rr|rr||rrr}
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Time}}} & \multicolumn{2}{c}{log(AF) = -0.20} & \multicolumn{2}{|c||}{log(AF) = 0} & \multicolumn{3}{c}{Average} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c||}{$H_0$} & 
    \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{$H_1$} & \multicolumn{1}{c}{$H_0$ or $H_1$} \\
    \hline
    BMA  & 5.3 (0.14) & 4.0.0 (--) & 10.6 (0.36) & 7.0 (0.96) & 7.8 (0.21) & 6.9 (0.93) & 7.8 (0.20) \\ 
    BF   & 5.6 (0.15) & 4.0.0 (--) & 11.4 (0.41) & 8.1 (0.97) & 8.3 (0.23) & 7.9 (0.95) & 8.3 (0.22) \\ 
    AIC  & 8.5 (0.18) & 0.0 (--) & 19.6 (0.52) & 29.3 (4.60) & 13.9 (0.32) & 29.3 (4.60) & 14.1 (0.33) \\ 
    BIC  & 8.4 (0.18) & 0.0 (--) & 19.6 (0.52) & 29.0 (4.57) & 13.8 (0.32) & 29.0 (4.57) & 14.0 (0.33) \\ 
    \hline
    \\
    
    \multicolumn{1}{l}{\multirow{2}{*}{\textbf{Time}}} & \multicolumn{2}{c}{log(AF) = 0.20} & \multicolumn{2}{|c||}{log(AF) = 0.40} & \multicolumn{3}{c}{Average} \\
    & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c|}{$H_1$} & \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c||}{$H_0$} & 
    \multicolumn{1}{|c}{$H_0$} & \multicolumn{1}{c}{$H_1$} & \multicolumn{1}{c}{$H_0$ or $H_1$} \\
    \hline
    BMA  & 11.1 (0.76) & 14.0 (0.55) & 7.8 (1.31) & 8.7 (0.27) & 10.8 (0.71) & 10.8 (0.29) & 10.8 (0.27) \\ 
    BF   & 11.6 (0.89) & 13.9 (0.54) & 8.8 (1.31) & 8.7 (0.26) & 11.4 (0.82) & 10.8 (0.28) & 10.9 (0.27) \\ 
    AIC  & 29.7 (2.15) & 28.5 (0.71) & 12.5 (5.07) & 16.9 (0.32) & 28.8 (2.11) & 21.6 (0.40) & 22.1 (0.40) \\  
    BIC  & 28.9 (2.08) & 28.3 (0.72) & 11.9 (5.57) & 16.6 (0.33) & 28.1 (2.05) & 21.4 (0.40) & 21.9 (0.41) \\ 
    \hline
\end{tabular}

\end{sidewaystable}
